An Epigraphical Approach to the Representer Theorem

Describing the solutions of inverse problems arising in signal or image processing is an important issue both for theoretical and numerical purposes. We propose a principle which describes the solutions to convex variational problems involving a finite number of measurements. We discuss its optimality on various problems concerning the recovery of Radon measures.

==> fig-epiR.tex <==



%% Regulariseur
\def\a{0.7} % main slope 
\def\xshift{2} % 
\def\altface{1.8} % altitude max de la face
\def\minregyface{0.7} % profondeur min de la face
\def\maxregyface{0.6*\k} % profondeur min de la face

%Face principale
\coordinate  (c0) at (\xshift+\a*\altface,\minregyface,\altface){};
\coordinate  (c1) at (\xshift+\a*\altface,\maxregyface,\altface){};
\coordinate  (c2) at (\xshift,\maxregyface,0){};
\coordinate  (c3) at (\xshift,\minregyface,0){};
%\draw[regcolor,dotted] (c0) -- (c1) -- (c2) -- (c3) --  cycle; 
\draw[regcolor,opacity=0.3]  (c1) -- (c2) ; 
\fill[regcolor!80, opacity=0.5] (c0) -- (c1) -- (c2) -- (c3) --  cycle; 

%Face du dessous 
\def\b{1.5} % lower slope^-1 
\def\altface{0.6} % altitude max de la face
  \coordinate  (c3do) at ($ (c3) + (-\b*\altface,0,-\altface) $){};
  \coordinate  (c2do) at ($ (c2) + (-\b*\altface,0,-\altface) $){};
\fill[regcolor!80,opacity=0.3] (c3do) -- (c3) -- (c2) -- (c2do) --  cycle; 
\draw[regcolor!80,opacity=0.1] (c3do) -- (c3) -- (c2) -- (c2do) --  cycle; 

% Face du dessus
\def\c{0.3} % upper slope^-1 
\def\altface{0.6} % altitude max de la face
\def\addy{0.3} 
  \coordinate  (c0up) at ($ (c0) + (\c*\altface,0,\altface) $){};
  \coordinate  (c1up) at ($ (c1) + (\c*\altface,0,\altface) $){};
  \fill[regcolor!80,opacity=0.3] (c0) -- (c0up) -- (c1up) -- (c1) --  cycle; 
  \draw[regcolor!80,opacity=0.1] (c0) -- (c0up) -- (c1up) -- (c1) --  cycle; 

%Face du dessous gauche
 \coordinate  (c3le) at ($ (c3do) + (0,-\addy,\altface) $){};
 \coordinate  (c2ri) at ($ (c2do) + (0,\addy,\altface) $){};
\fill[regcolor!80,opacity=0.1] (c3do) -- (c3le) -- (c3) -- cycle;
%\draw[regcolor!80,opacity=0.3,dotted] (c3do) -- (c3le) -- (c3) -- cycle;
\draw[regcolor!80,opacity=0.1] (c3do) -- (c3le) ;
%\fill[regcolor!80,opacity=0.3] (c2do) -- (c2ri) -- (c2) -- cycle;

%Face de gauche 
  \coordinate  (c0le) at ($ (c0) + (-\a*1.8-\b*\altface,-\addy,0) $){};
\draw[regcolor!80,opacity=0.1] (c0) -- (c3) -- (c3le) -- (c0le) -- cycle;
\fill[regcolor!80,opacity=0.1] (c0) -- (c3) -- (c3le) -- (c0le) -- cycle;

%Face dessus gauche
\def\altface{0.6} % altitude max de la face
  \coordinate  (c0leup) at ($ (c0le) + (0,0,\altface) $){};
%\draw[regcolor!80,opacity=0.3,dotted] (c0) -- (c0up) -- (c0leup) -- (c0le) -- cycle;
\draw[regcolor!80,opacity=0.1] (c0up) -- (c0leup) -- (c0le) ;
\fill[regcolor!80,opacity=0.1] (c0) -- (c0up) -- (c0leup) -- (c0le) -- cycle;


\draw[regcolor] (c0leup) node[below right] {$\epir=\epi(\reg)$};
%\draw[regcolor] (c0) node[below right] {$\face{\vecreg{p}}{\epir}$};



==> fig-hypof.tex <==
%%%Fidelity 
\def\minfidyface{0} % profondeur min de la face
\def\maxfidyface{\k} % profondeur min de la face
%Face principale
\def\minfidzface{0.3} % altitude min de la face
\def\maxfidzface{0.7} % altitude min de la face

\coordinate  (d0) at (\xshift+\a*\maxfidzface,\minfidyface,\maxfidzface){};
\coordinate  (d1) at (\xshift+\a*\minfidzface,\minfidyface,\minfidzface){};
%debug
%\draw (d0) node {$d_0$};
%\draw (d1) node {$d_1$};
%\draw[fidcolor!80, opacity=0.7,dotted] (d0) -- (d1); 

\def\upslope{0.5} % lower slope 
\def\xlength{1} %
\coordinate  (d0up) at ($ (d0) + (\xlength,0 ,\upslope*\xlength) $){};
\coordinate  (d0upright) at ($ (d0up) + (\xlength,0 ,0.25*\upslope*\xlength) $){};
%\coordinate  (d1do) at ($ (d1) + (-0.1\xlength,0 ,-\xlength) $){};
\coordinate  (d1do) at ($ (d1) + (-0.1\xlength,0 ,\zo-\minfidzface) $){};
%\draw[fidcolor!80, opacity=0.7,dotted] (d0upright) -- (d0up) -- (d0) -- (d1) -- (d1do); 


\coordinate  (e0upright) at ($ (d0upright) + (0,\maxfidyface-\minfidyface ,0) $){};
\coordinate  (e0up) at ($ (d0up) + (0,\maxfidyface-\minfidyface ,0) $){};
\coordinate  (e0) at ($ (d0) + (0,\maxfidyface-\minfidyface ,0) $){};
\coordinate  (e1do) at ($ (d1do) + (0,\maxfidyface-\minfidyface ,0) $){};
\coordinate  (e1) at ($ (d1) + (0,\maxfidyface-\minfidyface ,0) $){};

\coordinate  (elow) at ($ (e1do) + (2.1*\xlength+\a*\maxfidzface-\a*\minfidzface,0,0) $){};
\coordinate  (dlow) at ($ (d1do) + (2.1*\xlength+\a*\maxfidzface-\a*\minfidzface,0,0) $){};

\fill[fidcolor!80, opacity=0.1]   (elow) -- (dlow) -- (d1do) -- (e1do) -- cycle;
\fill[fidcolor!80, opacity=0.1] (d0upright) -- (d0up) -- (e0up) -- (e0upright) -- cycle;
\fill[fidcolor!80, opacity=0.1]  (d0up) -- (e0up) -- (e0) -- (d0) -- cycle;
\fill[fidcolor!80, opacity=0.4]   (e0) -- (d0) -- (d1) -- (e1) -- cycle;
\fill[fidcolor!80, opacity=0.1]   (d1) -- (e1) -- (e1do) -- (d1do) -- cycle;


\draw[fidcolor!80, opacity=0.05]  (elow) -- (e1do) -- (e1) -- (e0) -- (e0up) -- (e0upright) -- cycle;
%\draw (elow) node {elow}; % debug
\fill[fidcolor!80, opacity=0.1]   (elow) -- (e1do) -- (e1) -- (e0) -- (e0up) -- (e0upright) -- cycle;
\fill[fidcolor!80, opacity=0.1]   (dlow) -- (d1do) -- (d1) -- (d0) -- (d0up) -- (d0upright) -- cycle;
\fill[fidcolor!80, opacity=0.18]   (dlow) -- (d0upright) -- (e0upright) -- (elow) -- cycle;

\draw[fidcolor!80, opacity=0.2] (d0upright) -- (e0upright);
\draw[fidcolor!80, opacity=0.2] (d0up) -- (e0up);
\draw[fidcolor!80, opacity=0.2] (d0) -- (e0);
\draw[fidcolor!80, opacity=0.2] (d1) -- (e1);
%\draw[fidcolor!80, opacity=0.2] (d1do) -- (e1do);

\draw[fidcolor!80, opacity=0.1]  (dlow) -- (d1do) -- (d1) -- (d0) -- (d0up) -- (d0upright) -- cycle;

\draw[fidcolor] (elow) node[xshift=-40,yshift=20] {$\hypof=\hypo(\minval-\fidp)$};


